Automatic analysis of distance bounding protocols

Distance bounding protocols are used by nodes in wireless networks to calculate upper bounds on their distances to other nodes. However, dishonest nodes in the network can turn the calculations both illegitimate and inaccurate when they participate in protocol executions. It is important to analyze protocols for the possibility of such violations. Past efforts to analyze distance bounding protocols have only been manual. However, automated approaches are important since they are quite likely to find flaws that manual approaches cannot, as witnessed in literature for analysis pertaining to key establishment protocols. In this paper, we use the constraint solver tool to automatically analyze distance bounding protocols. We first formulate a new trace property called Secure Distance Bounding (SDB) that protocol executions must satisfy. We then classify the scenarios in which these protocols can operate considering the (dis)honesty of nodes and location of the attacker in the network. Finally, we extend the constraint solver so that it can be used to test protocols for violations of SDB in these scenarios and illustrate our technique on some published protocols.

==> extension.tex <==
\subsection{Defining Secure Distance Bounding}

Our aim is to find out if a protocol can be subverted such that a node can be shown as being at a false distance. We will say that a protocol satisfies the property of Secure Distance Bounding (SDB) if such a subversion is not possible on the protocol.

To extend constraint solving to test for the violation of the Secure Distance Bounding (SDB) property, we need to first define the property and the protocol execution scenario(s) when we consider it violated.

At first sight, such an extension seems complicated since we might have to use a \underline{timed} model which is not used by most protocol analysis tools to date including the constraint solver. Fortunately, that is not the case since the SDB property can be so defined such that whether the main goal of the protocol is reached or not can be tested using purely the ability of the attacker to generate messages (similar to testing secrecy and authentication).

It is easier to analyze a distance bounding protocol by splitting it into two parts:

\begin{enumerate}

	\item The distance bounding part;
	\item The authentication part.

\end{enumerate}

 The distance bounding part usually involves a challenge-response mechanism, while authentication (with or without key exchange) can occur before or after the distance bounding part.

Informally, an attack on a distance bounding protocol exists if the attacker can finish the distance bounding part (by sending the response to the challenge) and the authentication part by sending the messages in that part such as MACs and Signatures. For instance, the circled portion in Figure~\ref{f.P3} indicates the rapid-response and the MAC in protocol \textbf{P3} to be sent to the verifier to finish the protocol.

\begin{figure}[h]
\centering
\scalebox{.40}
{\includegraphics*[viewport=85 455 520 725]{P4.pdf}}
\caption{Protocol P3 execution}\label{f.P3}
\end{figure}

It is difficult to formalize this concept since not all protocols fall necessarily into the above model with two parts. For example, the Echo protocol does not in fact have an authentication part. There could be other protocols that exist at present or in the future that may not have the rapid response part. Hence, we will have a general definition for an attack that at least covers all the protocols considered in this paper:

\begin{definition}\label{d.SDB}
	
	If an attacker can synthesize the rapid-response and finish a protocol then an attack (or a violation) of SDB property is possible on the protocol.

\end{definition}

However, there is a big glitch in this definition: virtually all the protocols  \textbf{P1} through \textbf{P5} (and possibly other protocols in literature) as well will have a straightforward attack wherein the attacker is in between $P$ and $V$ responds as `$p$' in the non-authentic distance bounding part and relays $p$'s messages to $v$ in the authentication part (see Figure \ref{f.Relay}).

\begin{figure}[h]
\centering
\scalebox{.40}
{\includegraphics*[viewport=85 665 400 715]{Relay.pdf}}
\caption{i spoofing as p making it appear closer by relaying messages}\label{f.Relay}
\end{figure}

Indeed, that is a scenario with an attacker between the prover and verifier and hence will be able to fake that the prover is closer to the verifier. This can happen with the help of the prover or without (using wormholes) and are termed ``collusion attacks". It is a known problem to which all distance bounding protocols are susceptible and to which a solution is not yet known \cite{MPPCS07}.

Since collusion attacks are anyway not preventable except through ``best-effort" solutions such as periodic identification and elimination of dishonest nodes \cite{MPPCS07}, we will look at other classes of attacks where collusion does not take place, namely:

\begin{enumerate}

\item \textbf{Pure attacker} scenario (there is no prover strand);

\item \textbf{Pure dishonest prover} scenario (the prover could be a legitimate machine but no collusion with other nodes is involved); and

\item \textbf{Attacker and honest prover} scenario (no collusion);

\end{enumerate}

The only other scenario is the most powerful scenario with full collusion as explained above. 

Note that it is always possible to pretend that the prover is further away by simply delaying the rapid-response. This can be prevented by localization protocols such as SPINE that uses triangulation \cite{CH06} or most recently protocols that satisfy the SDM (Secure Distance Modification) property which uses multiple provers to localize a verifier that is not necessarily enclosed by the provers \cite{SW07}.  Hence, we will not consider attacks with distance enlargement in our analysis in this paper.

\section{Analyzing \textbf{P1} to \textbf{P5}}

Let us start with protocol \textbf{P1}. We can analyze this protocol with one strand per role and find the simple attack:

\begin{figure}[h]
\centering
\scalebox{0.7}
{\includegraphics*[viewport=75 633 350 715]{P1-Attack1.pdf}}
\caption{Attack on \textbf{P1}; pure attacker setting}\label{f.P1-Attack}
\end{figure}

Obviously, this attack exists with a ``pure attacker" scenario with no one playing `$P$'. It is interesting to ask whether an attack exists with a dishonest agent playing `$P$', but no attacker. i.e. `$p$' is not spoofing anyone, but is attempting to pretend being closer to `$v$'. Following Def.~\ref{d.SDB}, we need to determine if it is possible for the (dishonest) `$p$' to send the rapid-response and finish the protocol. Hence, we need to create a constraint sequence with just the second message as:

\begin{center}  

	$p~:~\{v, p, i \}$

\end{center}

\noindent
which is solvable. Hence, there is an attack in this sequence where `$p$' just jumps the gun before recieving Msg 1 from $v$:

\begin{figure}[h]
\centering
\scalebox{0.8}
{\includegraphics*[viewport=50 650 325 715]{P1-Attack2.pdf}}
\caption{Attack on \textbf{P1}; pure dishonest prover setting}\label{f.P1-Attack}
\end{figure}

The Echo protocol \textbf{P2} can be subject to a similar analysis. It has essentially the same attack as above on \textbf{P1} in a pure-attacker setting:

\begin{figure}[h]
\centering
\scalebox{0.7}
{\includegraphics*[viewport=75 633 350 715]{P2-Attack.pdf}}
\caption{Attack on \textbf{P2} (\textbf{Echo}); pure attacker setting}\label{f.P2-Attack}
\end{figure}

However, there is no attack in a ``pure dishonest prover" setting, since the constraint

\begin{center}  

$n_v~:~\{ v, p, i \}$

\end{center}

\noindent
cannot be solved without $n_v$ in the term set. Agent `$p$', no matter how much it wishes it doesn't, will have to wait to recieve Msg 1 from wherever it is at.

Protocol \textbf{P3} can be analyzed similar to \textbf{P2} but with the addition of the authenticated Msg 3. An attack cannot be formed without any verifier strand since Msg 3 cannot be synthesized by an attacker. However, there is an attack with just one strand each for the prover and verifier, where the attacker responds with the rapid-response and then simply relays Msg 3 but this is a collusion attack that we are less interested in:

\begin{center}
\begin{tabular}{ll}

Msg 1. $v \to i : n_v$ \\

Msg 2. $i \to v : n_v$\\

Msg 3. $p \to v : \mi{Sig}_{\mi{pk}(p)}(h(n_v, v, p))$\\

\end{tabular}
\end{center}


\begin{figure}[h]
\centering
\scalebox{.35}
{\includegraphics*[viewport=85 475 520 725]{P3-Attack1.pdf}}
\caption{Attack1 on \textbf{P3}}\label{f.P3-Attack1}
\end{figure}

This attack can be visualized when we solve the constraint sequence:

\begin{center}
\begin{eqnarray*}
N_V & : & \{ n_i, v, p \}~~~(= T_0) \\
n_v & : & \{ n_v \} \cup T_0~~~(= T_1) \\
\mi{Sig}_{\mi{pk}(P)}(h(n_v, v, P)) & : & \{ \mi{Sig}_{\mi{pk}(p)}(h(N_V, v, P)) \} \cup  T_1
\end{eqnarray*}
\end{center}

The first constraint can be skipped since it has only a variable on the left (a ``simple" constraint) and the second is obviously satisfiable, leaving us with only the last constraint which is satisfiable through unification of the signature terms.

Switching the first and second constraints above reveals another attack on \textbf{P3}. In this scenario, the attacker spoofs as $p$ to $v$ and vice-versa (there is no collusion with $v$):

\begin{center}
\begin{tabular}{ll}

Msg $\alpha$.1. $v \to i(p) : n_v$ \\

Msg $\alpha$.2. $i(p) \to v : n_v$\\

~~~Msg $\beta$.1. $i(v) \to p : n_v$ \\

~~~Msg $\beta$.2. $p \to i(v) : n_v$ \\

~~~Msg $\beta$.3. $p \to i(v) : \mi{Sig}_{\mi{pk}(p)}(h(n_v, v, p))$\\

Msg $\alpha$.3. $i(p) \to v : \mi{Sig}_{\mi{pk}(p)}(h(n_v, v, p))$~~~(Replaying Msg $\beta$.3)\\ 

\end{tabular}
\end{center}


\begin{figure}[h]
\centering
\scalebox{.35}
{\includegraphics*[viewport=85 400 520 725]{P3-Attack2.pdf}}
\caption{Attack2 on \textbf{P3}}\label{f.P3-Attack2}
\end{figure}

Note that this attack cannot exist if there was a field, say `$POS_P$' (denoting $P$'s position) that is paired in Msg 2 and inside the signature in Msg 3. In this case, the constraints would be:

\begin{center}
\begin{eqnarray*}
[ n_v, POS_p] & : & \{ n_v, v, p \}~~~(= T_0) \\ 
N_V & : & T_0 \\
\mi{Sig}_{\mi{pk}(p)}( h(n_v, v, p, POS_p)) & : & \mi{Sig}_{\mi{pk}(p)}(h(N_V, v, p, pos_p)) \cup T_0 
\end{eqnarray*}
\end{center}

It is not possible to solve this sequence with a different value for $POS_P$ in Msg 2 compared to Msg 3 since the first constraint could be split into $n_v~:~\{ n_v, v, p \}$ (which is solvable) and $POS_p~:~\{ n_v, v, p \}$ (which is skipped since it is a simple constraint). That leaves us with the last constraint which assigns the value of $pos_p$ for $POS_p$ when unifying the signatures on the left and right sides. Hence, $i$ can convince $a$ of an incorrect distance from $b$ only if $b$ colludes with $i$ and produces a signed message with the incorrect distance.

Protocol \textbf{P4} also has an obvious collusion attack but none with just the verifier and attacker. With one strand each for the verifier and prover, a Man-in-the-Middle (MITM) attack but without collusion is possible as shown in the figure below:

\begin{figure}[h]
\centering
\scalebox{.35}
{\includegraphics*[viewport=85 350 520 725]{P4-Attack.pdf}}
\caption{MITM attack on \textbf{P4}}\label{f.P4-Attack}
\end{figure}

The most relevant constraints in the sequence generated for this attack are as follows:

\begin{center}
\begin{eqnarray*}
N_P & : & \{ n_i, v, p, i \}~~~(= T_0) \\
N_V & : & \{ n_v, n_p \} \cup T_0~~~(= T_1) \\
n_v \oplus N_P & : & \{ N_V \oplus n_p \} \cup T_1~~~(= T_2) \\
\lefteqn{[}~n_v , v, p]_{\mi{sh}(v,p)} & : & \{ [ N_V, v, p ]_{\mi{sh}(v,p)} \} \cup T_2
\end{eqnarray*}
\end{center}

It is possible to avoid this attack by simply requiring the prover's nonce in the MAC (Msg 5). In that case, the last constraint becomes, \\

$[n_v , v, p, N_P]_{\mi{sh}(v,p)} : \{ [ N_V, v, p, n_p ]_{\mi{sh}(v,p)} \} \cup T_2$ \\

\noindent
which is not solvable through unification of the encryptions on both sides if the first constraint was solved by substituting any other value for $N_P$ than $n_p$. Indeed, that has to be the case since there is no $n_p$ in the term set of the first constraint.

%Note that including agent identities and/or component numbers (following the most widely successful prudent engineering practices \cite{AN94, Lowe96} for preventing parallel-run attacks) is not sufficient.

It turns out that both flaws in \textbf{P3} and \textbf{P4} have been corrected in \textbf{P5} by including the $POS_P$ field and the prover's nonce $N_P$ in the MAC. Thus it avoids both the attacks demonstrated on \textbf{P3} and \textbf{P4} (It is however vulnerable to collusion attacks like all other distance bounding protocols as explained in \cite{MPPCS07}).     

Note that an attack does not necessarily exist whenever Def \ref{d.SDB} is satisfied. For instance, consider the following scenario between a verifier, attacker and prover:

\begin{figure}[h]
\centering
\scalebox{.35}
{\includegraphics*[viewport=75 340 520 725]{P5-Attack.pdf}}
\caption{(Not a) MITM attack on \textbf{P5}}\label{f.P5-Attack}
\end{figure}

This is a possible execution of \textbf{P5} assuming an honest prover. In this case, both the rapid-response and the authenticated response have been satisfied, yet in reality there is no attack since $i(p)$ has to send the rapid-response \emph{immediately} after recieving the request (Msg 2). This is required to satisfy the time constraints in sensor networks. $i(p)$ cannot wait to hear Msg 3 from $p$ to send its response to $v$ in turn, especially if it is trying to lie about $p$ being closer than it atually is. This means that our definition is complete but not sound. We conduct our analyses by trying to determine if all messages in the verifier strand can be synthesized. A positive outcome will not mean an attack but at least we do not lose any attack. 
